Nested Sequents for First-Order Modal Logics via Reachability Rules

We introduce the first cut-free nested sequent systems for first-order modal logics that admit increasing, decreasing, constant, and empty domains along with so-called general path conditions and seriality. We obtain such systems by means of two devices: 'reachability rules' and 'structural refinement'. Regarding the former device, we introduce reachability rules as special logical rules parameterized with formal grammars (viz. types of semi-Thue systems) that operate by propagating formulae and/or checking if data exists along certain paths within a nested sequent, where paths are encoded as strings generated by a parameterizing grammar. Regarding the latter device, structural refinement is a relatively new methodology used to extract nested sequent systems from labeled systems (which are ultimately obtained from a semantics) by means of eliminating structural/relational rules, introducing reachability rules, and then carrying out a notational translation. We therefore demonstrate how this method can be extended to the setting of first-order modal logics, and expose how reachability rules naturally arise from applying this method.

==> app-proofs.tex <==



 In this appendix, we provide two lemmata sufficient to conclude the completeness of our labeled calculi. First, we define a semantics for labeled sequents, interpreting them over models for first-order modal logics.
 
 
\begin{definition}[Labeled Sequent Semantics] Let $\fcset$ be a set of frame conditions and $M = (W,R,D,V)$ a model based on a frame $F \in \mathcal{F}_{\fcset}$. We define an \emph{$M$-interpretation} to be a function $\iota : \lab \to W$. Satisfaction for a multiset $\rel$ of relational and domain atoms, or a multiset $\Gamma$ of labeled formulae, is defined accordingly:
\begin{itemize}

\item $M,\mu,\iota \models \rel$ \iffi for each $wRu, x \in D(w) \in \rel$, $(\iota(w),\iota(u)) \in R$ and $\mu(x) \in D(\iota(w))$;

\item $M,\mu,\iota \models \Gamma$ \iffi for each $w : \phi \in \Gamma$, $M,\iota(w),\mu \Vdash \phi$.

\end{itemize}
 We say that a labeled sequent $\Lambda = \rel, \Gamma \sar \Delta$ is \emph{satisfied} on $M$ with $\mu$ and $\iota$, written $M,\mu,\iota \models \Lambda$, \iffi if $M,\mu,\iota \models \rel$ and $M,\mu,\iota \models \Gamma$, then there exists a $w : \phi \in \Delta$ such that $M,\mu,\iota \models w : \phi$. We define a labeled sequent to be \emph{$\fcset$-valid} \iffi for every model $M$ based on a frame in $\mathcal{F}_{\fcset}$, every $M$-assignment $\mu$, and every $M$-interpretation $\iota$, $M,\mu,\iota \models \Lambda$, and we say that $\Lambda$ is \emph{$\fcset$-invalid}, and write $M,\mu,\iota \not\models \Lambda$, otherwise.
\end{definition}

 The following lemma is easily shown by induction on the height of a derivation ending with an application of $\neu$, and follows from the fact that $\neu$ can be absorbed into instances of $\ax$ and permuted with all other rules of $\lql$.

\begin{lemma}\label{lem:neu-admiss}
The $\neu$ rule (shown below) is hp-admissible in $\lql$:
\begin{center}
\AxiomC{$\rel, x \in D(w), \Gamma \sar \Delta$}
\RightLabel{$\neu^{\dag}$}
\UnaryInfC{$\rel, \Gamma \sar \Delta$}
\DisplayProof
\end{center}
 where the side condition $\dag$ stipulates that the rule is applicable only if $x$ and $w$ are fresh.
\end{lemma}



 We define a \emph{pseudo-derivation} to be a (potentially infinite) structure obtained by bottom-up applying the rules of $\lql$ to a given labeled sequent (which serves as the conclusion of the pseudo-derivation). Observe that every proof is a pseudo-derivation where all top sequents are instances of the $\ax$ rule. We define a \emph{branch} $\branch$ in a pseudo-derivation to be a path of labeled sequents satisfying: (1) the conclusion of the pseudo-derivation is the $1^{st}$ element of the path, (2) if a labeled sequent $\Lambda$ in the pseudo-derivation is the $n^{th}$ element in the path and is not an instance of $\ax$, then one of the premises of $\Lambda$ is the $(n+1)^{th}$ element of the path. % maximal, linear path of labeled sequents starting from the conclusion and continuing upward through the pseudo-derivation.

 
 
\begin{lemma}
If $\Lambda$ is $\fcset$-valid, then $\Lambda$ is provable in $\lql$.
\end{lemma}

\begin{proof} Let $\Lambda = \rel, \Gamma \sar \Delta$ such that $\Gamma \cup \Delta \neq \emptyset$ and suppose that $\Lambda$ is not provable in $\lql$. We may assume w.l.o.g. that $\Gamma \cup \Delta \neq \emptyset$ since if both $\Gamma$ and $\Delta$ are empty, then $\Lambda$ is $\fcset$-invalid. Let $y$ be a variable not occurring in $\Lambda$ and $u$ be a label not occurring in $\Lambda$. We let $\Lambda' = \rel, y \in D(u), \Gamma \sar \Delta$. We now define a (potentially non-terminating) proof search procedure $\prove$, and show that if $\prove$ does not terminate, then a counter-model $M$ for $\Lambda$ based a frame in $F \in \mathcal{F}_{\fcset}$ can be extracted.\\

\noindent
$\prove$. We take $\Lambda'$ as input and proceed to the $\ax$ step below.\\

\noindent
$\ax$. Let $\branch_{1}, \ldots, \branch_{n}$ be all branches in the pseudo-derivation so far constructed with $\Lambda_{1}, \ldots, \Lambda_{n}$ the top sequents of each branch, respectively. For each $\Lambda_{i}$ that is an instance of $\ax$, halt $\prove$. If $\prove$ has halted on $\branch_{i}$ for each $1 \leq i \leq n$, then return $\true$. If $\prove$ has not halted on $\branch_{i}$ for each $1 \leq i \leq n$, then let $\branch_{j_{1}}, \ldots, \branch_{j_{k}}$ be all branches for which $\prove$ did not halt. For each of these branches, copy the top sequent above itself, and continue to the next step.

\medskip

\noindent
$\negl$. Let $\branch_{1}, \ldots, \branch_{n}$ be all branches in the pseudo-derivation so far constructed with $\Lambda_{1}, \ldots, \Lambda_{n}$ the top sequents of each branch, respectively. We successively consider each branch. Suppose that $\branch_{1}, \ldots, \branch_{k}$ have already been considered. Let $\Lambda_{k+1}$ be of the form:
$$
\rel, \Gamma, w_{1} : \neg \phi_{1}, \ldots, w_{m} :\neg \phi_{m} \sar \Delta
$$
 with $w_{1} : \neg \phi_{1}, \ldots, w_{m} :\neg \phi_{m}$ all negated formulae in the antecedent of $\Lambda_{k+1}$. We successively consider each negated formula and apply $\negl$ bottom-up in each case. This extends $\branch_{k+1}$ so that it now has a top-sequent of the form:
$$
\rel, \Gamma \sar w_{1} : \phi_{1}, \ldots, w_{m} :\phi_{m}, \Delta
$$
 Once every branch has been considered, continue to the next step.
 
\medskip

\noindent
$\negr$. Let $\branch_{1}, \ldots, \branch_{n}$ be all branches in the pseudo-derivation so far constructed with $\Lambda_{1}, \ldots, \Lambda_{n}$ the top sequents of each branch, respectively. We successively consider each branch. Suppose that $\branch_{1}, \ldots, \branch_{k}$ have already been considered. Let $\Lambda_{k+1}$ be of the form:
$$
\rel, \Gamma \sar w_{1} : \neg \phi_{1}, \ldots, w_{m} :\neg \phi_{m}, \Delta
$$
 with $w_{1} : \neg \phi_{1}, \ldots, w_{m} :\neg \phi_{m}$ all negated formulae in the consequent of $\Lambda_{k+1}$. We successively consider each negated formula and apply $\negr$ bottom-up in each case. This extends $\branch_{k+1}$ so that it now has a top-sequent of the form:
$$
\rel, \Gamma, w_{1} : \phi_{1}, \ldots, w_{m} :\phi_{m} \sar \Delta
$$
 Once every branch has been considered, continue to the next step.

\medskip


%%%DISL
\noindent
$\disl$. Let $\branch_{1}, \ldots, \branch_{n}$ be all branches in the pseudo-derivation so far constructed with $\Lambda_{1}, \ldots, \Lambda_{n}$ the top sequents of each branch, respectively. We successively consider each branch. Suppose that $\branch_{1}, \ldots, \branch_{k}$ have already been considered. Let $\Lambda_{k+1}$ be of the form:
$$
\rel, \Gamma, w_{1} : \phi_{1} \lor \psi_{1}, \ldots, w_{m} : \phi_{m} \lor \psi_{m} \sar \Delta
$$
 with $w_{1} : \phi_{1} \lor \psi_{1}, \ldots, w_{m} : \phi_{m} \lor \psi_{m}$ all disjunctive formulae in the antecedent of $\Lambda_{k+1}$. We successively consider each disjunctive formula and apply the $\disl$ rule bottom-up. This yields $2^{m}$ new branches extending $\branch_{k+1}$, each having a top labeled sequent of the form:
$$
\rel, \Gamma, w_{1} : \chi_{1}, \ldots, w_{m} :\chi_{m} \sar \Delta
$$
 where $\chi_{i} \in \{\phi_{i},\psi_{i}\}$ for $1 \leq i \leq n$. Once every branch has been considered, continue to the next step.
 
\medskip


%%%DISR
\noindent
$\disr$. Let $\branch_{1}, \ldots, \branch_{n}$ be all branches in the pseudo-derivation so far constructed with $\Lambda_{1}, \ldots, \Lambda_{n}$ the top sequents of each branch, respectively. We successively consider each branch. Suppose that $\branch_{1}, \ldots, \branch_{k}$ have already been considered. Let $\Lambda_{k+1}$ be of the form:
$$
\rel, \Gamma \sar w_{1} : \phi_{1} \lor \psi_{1}, \ldots, w_{m} : \phi_{m} \lor \psi_{m}, \Delta
$$
 with $w_{1} : \phi_{1} \lor \psi_{1}, \ldots, w_{m} : \phi_{m} \lor \psi_{m}$ all disjunctive formulae in the consequent of $\Lambda_{k+1}$. We successively consider each disjunctive formula and apply the $\disr$ rule bottom-up. This yields a new branch extending $\branch_{k+1}$, so that it now has a top labeled sequent of the form:
$$
\rel, \Gamma \sar w_{1} : \phi_{1}, w_{1} : \psi_{1}, \ldots, w_{m} : \phi_{m}, w_{m} : \psi_{m}, \Delta
$$
 Once every branch has been considered, continue to the next step.
 
\medskip


%%%DIAL
\noindent
$\dial$. Let $\branch_{1}, \ldots, \branch_{n}$ be all branches in the pseudo-derivation so far constructed with $\Lambda_{1}, \ldots, \Lambda_{n}$ the top sequents of each branch, respectively. We successively consider each branch. Suppose that $\branch_{1}, \ldots, \branch_{k}$ have already been considered. Let $\Lambda_{k+1}$ be of the form:
$$
\rel, \Gamma, w_{1} : \Diamond \phi_{1}, \ldots, w_{m} : \Diamond \phi_{m} \sar \Delta
$$
 with $w_{1} : \Diamond \phi_{1}, \ldots, w_{m} : \Diamond \phi_{m}$ all diamond formulae in the antecedent of $\Lambda_{k+1}$. We successively consider each diamond formula and apply the $\dial$ rule bottom-up. This yields a new branch extending $\branch_{k+1}$, so that it now has a top labeled sequent of the form:
$$
\rel, w_{1}Ru_{1}, \ldots, w_{m}Ru_{m}, \Gamma, u_{1} : \phi_{1}, \ldots, u_{m} : \phi_{m} \sar \Delta
$$
 with $u_{1}, \ldots, u_{m}$ fresh. Once every branch has been considered, continue to the next step.
 
\medskip


%%%DIAR
\noindent
$\diar$. Let $\branch_{1}, \ldots, \branch_{n}$ be all branches in the pseudo-derivation so far constructed with $\Lambda_{1}, \ldots, \Lambda_{n}$ the top sequents of each branch, respectively. We successively consider each branch. Suppose that $\branch_{1}, \ldots, \branch_{k}$ have already been considered. Let $\Lambda_{k+1}$ be of the form:
$$
\rel, \Gamma \sar w_{1} : \Diamond \phi_{1}, \ldots, w_{m} : \Diamond \phi_{m}, \Delta
$$
 with $w_{1} : \Diamond \phi_{1}, \ldots, w_{m} : \Diamond \phi_{m}$ all diamond formulae in the consequent of $\Lambda_{k+1}$. We successively consider each diamond formula $w_{i}: \Diamond \phi_{i}$ and each relational atom of the form $w_{i}Ru$ and apply the $\diar$ rule bottom-up. This yields a new branch extending $\branch_{k+1}$ with a top labeled sequent where all diamond formulae in the consequent have been `propagated.' Once every branch has been considered, continue to the next step.
 
\medskip


%%EXISTL
\noindent
$\existsl$. Let $\branch_{1}, \ldots, \branch_{n}$ be all branches in the pseudo-derivation so far constructed with $\Lambda_{1}, \ldots, \Lambda_{n}$ the top sequents of each branch, respectively. We successively consider each branch. Suppose that $\branch_{1}, \ldots, \branch_{k}$ have already been considered. Let $\Lambda_{k+1}$ be of the form:
$$
\rel, \Gamma, w_{1} : \exists x_{1} \phi_{1}, \ldots, w_{m} : \exists x_{m} \phi_{m} \sar \Delta
$$
 with $w_{1} : \exists x_{1} \phi_{1}, \ldots, w_{m} : \exists x_{m} \phi_{m}$ all existential formulae in the antecedent of $\Lambda_{k+1}$. We successively consider each existential formula and apply the $\existsl$ rule bottom-up. This yields a new branch extending $\branch_{k+1}$, so that it now has a top labeled sequent of the form:
$$
\rel, y_{1} \in D(w_{1}), \ldots, y_{m} \in D(w_{m}), \Gamma, w_{1} : \phi_{1}[y_{1}/x_{1}], \ldots, w_{m} : \phi_{m}[y_{m}/x_{m}] \sar \Delta
$$
 with $y_{1}, \ldots, y_{m}$ fresh. Once every branch has been considered, continue to the next step.
 
\medskip


%%EXISTR
\noindent
$\existsr$. Let $\branch_{1}, \ldots, \branch_{n}$ be all branches in the pseudo-derivation so far constructed with $\Lambda_{1}, \ldots, \Lambda_{n}$ the top sequents of each branch, respectively. We successively consider each branch. Suppose that $\branch_{1}, \ldots, \branch_{k}$ have already been considered. Let $\Lambda_{k+1}$ be of the form:
$$
\rel, \Gamma \sar w_{1} : \exists x_{1} \phi_{1}, \ldots, w_{m} : \exists x_{m} \phi_{m}, \Delta
$$
 with $w_{1} : \exists x_{1} \phi_{1}, \ldots, w_{m} : \exists x_{m} \phi_{m}$ all existential formulae in the consequent of $\Lambda_{k+1}$. We successively consider each existential formula $w_{i}: \exists x_{i} \phi_{i}$ and each domain atom of the form $y \in D(w_{i})$ and apply the $\existsr$ rule bottom-up. This yields a new branch extending $\branch_{k+1}$ with a top labeled sequent where all existential formulae in the consequent have been `instantiated.' Once every branch has been considered, continue to the next step.
 
\medskip

%%DOMR
\noindent
$\domr$. Let $\branch_{1}, \ldots, \branch_{n}$ be all branches in the pseudo-derivation so far constructed with $\Lambda_{1}, \ldots, \Lambda_{n}$ the top sequents of each branch, respectively. We successively consider each branch. Suppose that $\branch_{1}, \ldots, \branch_{k}$ have already been considered. Let $\Lambda_{k+1}$ be of the form:
$$
\rel, \Gamma, w_{1} : p_{1}(\vec{x}_{1}), \ldots, w_{m} : p_{m}(\vec{x}_{m}) \sar \Delta
$$
 with $w_{1} : p_{1}(\vec{x}_{1}), \ldots, w_{m} : p_{m}(\vec{x}_{m})$ all atomic formulae in the antecedent of $\Lambda_{k+1}$. We successively consider each atomic formula $w_{i} : p_{i}(\vec{x}_{i})$ and apply the $\domr$ rule bottom-up. This yields a new branch extending $\branch_{k+1}$ with a top labeled sequent of the form:
$$
\rel, \vec{x}_{i} \in D(w_{1}), \ldots, \vec{x}_{m} \in D(w_{m}), \Gamma, w_{1} : p_{1}(\vec{x}_{1}), \ldots, w_{m} : p_{m}(\vec{x}_{m}) \sar \Delta
$$
 Once every branch has been considered, continue to the next step.
 
\medskip


\noindent
$\D$. If $S \in \fcset$, then perform the following: Let $\branch_{1}, \ldots, \branch_{n}$ be all branches in the pseudo-derivation so far constructed with $\Lambda_{1}, \ldots, \Lambda_{n}$ the top sequents of each branch, respectively. We successively consider each branch. Suppose that $\branch_{1}, \ldots, \branch_{k}$ have already been considered. Let $\Lambda_{k+1} = \rel', \Gamma' \sar \Delta'$ be the top labeled sequent in $\branch_{k+1}$. For each $w \in \lab(\Lambda_{k+1})$, apply $\D$ bottom-up introducing $wRu$ with $u$ a fresh label. This yields a new branch extending $\branch_{k+1}$. Once every branch has been considered, continue to the next step.

\medskip

\noindent
$\sa$. If $G(n,k) \in \fcset$, then perform the following: Let $\branch_{1}, \ldots, \branch_{n}$ be all branches in the pseudo-derivation so far constructed with $\Lambda_{1}, \ldots, \Lambda_{n}$ the top sequents of each branch, respectively. We successively consider each branch. Suppose that $\branch_{1}, \ldots, \branch_{k}$ have already been considered. Let $\Lambda_{k+1} = \rel', \Gamma' \sar \Delta'$ be the top labeled sequent in $\branch_{k+1}$. For each sequence $wR^{n}u$ and $wR^{k}v$ of relational atoms in $\rel'$ apply $\sa$ bottom-up introducing $uRv$. This yields a new branch extending $\branch_{k+1}$. Once every branch has been considered, continue to the next step.

\medskip

\noindent
$\idom$. If $I_{d} \in \fcset$, then perform the following: Let $\branch_{1}, \ldots, \branch_{n}$ be all branches in the pseudo-derivation so far constructed with $\Lambda_{1}, \ldots, \Lambda_{n}$ the top sequents of each branch, respectively. We successively consider each branch. Suppose that $\branch_{1}, \ldots, \branch_{k}$ have already been considered. Let $\Lambda_{k+1} = \rel', \Gamma' \sar \Delta'$ be the top labeled sequent in $\branch_{k+1}$. For each pair $wRu, x \in D(w) \in \rel'$, apply $\idom$ bottom-up introducing $x \in D(u)$. This yields a new branch extending $\branch_{k+1}$. Once every branch has been considered, continue to the next step.

\medskip

\noindent
$\ddom$. If $D_{d} \in \fcset$, then perform the following: Let $\branch_{1}, \ldots, \branch_{n}$ be all branches in the pseudo-derivation so far constructed with $\Lambda_{1}, \ldots, \Lambda_{n}$ the top sequents of each branch, respectively. We successively consider each branch. Suppose that $\branch_{1}, \ldots, \branch_{k}$ have already been considered. Let $\Lambda_{k+1} = \rel', \Gamma' \sar \Delta'$ be the top labeled sequent in $\branch_{k+1}$. For each pair $wRu, x \in D(u) \in \rel'$, apply $\ddom$ bottom-up introducing $x \in D(w)$. This yields a new branch extending $\branch_{k+1}$. Once every branch has been considered, continue to the next step.

\medskip

\noindent
$\ned$. If $N_{d} \not\in \fcset$, then continue to the $\ax$ step. If $N_{d} \in \fcset$, then perform the following: Let $\branch_{1}, \ldots, \branch_{n}$ be all branches in the pseudo-derivation so far constructed with $\Lambda_{1}, \ldots, \Lambda_{n}$ the top sequents of each branch, respectively. We successively consider each branch. Suppose that $\branch_{1}, \ldots, \branch_{k}$ have already been considered. Let $\Lambda_{k+1} = \rel', \Gamma' \sar \Delta'$ be the top labeled sequent in $\branch_{k+1}$. For each $w \in \lab(\Lambda_{k+1})$, apply $\ned$ bottom-up introducing $y \in D(w)$ with $y$ fresh. This yields a new branch extending $\branch_{k+1}$. Once every branch has been considered, continue to the $\ax$ step.

\medskip

\noindent
This ends the description of $\prove$.\\

 If $\prove$ terminates, then the pseudo-derivation it constructs is a proof in $\lql$ with the conclusion $\Lambda' = \rel, y \in D(u), \Gamma \sar \Delta$. Observe that applying the $\neu$ rule a single time, yields a proof of $\Lambda$ in $\lql$, as $\neu$ can be eliminated by \lem~\ref{lem:neu-admiss} above. Note that $\neu$ is applicable as $y$ and $u$ do not occur in $\Lambda$. Therefore, we have a contradiction as $\Lambda$ was assumed to not have a proof in $\lql$, and thus, $\prove$ does not terminate. Hence, $\prove$ constructs an infinite pseudo-derivation, which is finitely branching, and so by K\"onig's lemma, an infinite branch $\branch$ must exist in the pseudo-derivation. We let $\Lambda'' \in \branch$ mean that the labeled sequent $\Lambda''$ occurs in the branch $\branch$, and define the following:
$$
\mathbf{R} = \!\!\!\!\!\!\!\! \bigcup_{\rel', \Gamma' \sar \Delta' \in \branch} \!\!\!\!\!\!\!\! \rel'
\qquad
\mathbf{\Gamma} = \!\!\!\!\!\!\!\! \bigcup_{\rel', \Gamma' \sar \Delta' \in \branch} \!\!\!\!\!\!\!\! \Gamma'
\qquad
\mathbf{\Delta} = \!\!\!\!\!\!\!\! \bigcup_{\rel', \Gamma' \sar \Delta' \in \branch} \!\!\!\!\!\!\!\! \Delta'
$$
 We now define a model $M = (W,R,D,V)$ as shown below:
\begin{itemize}

\item $W = \lab(\mathbf{R},\mathbf{\Gamma},\mathbf{\Delta})$;

%\item $x \in U$ \iffi there exists a $w \in \lab(\mathbf{R},\mathbf{\Gamma},\mathbf{\Delta})$ such that $x \in D(w) \in \mathbf{R}$, or there exists a $w : p(\vec{x}) \in \mathbf{\Gamma}$ with $x \in \vec{x}$;

\item $(w,u) \in R$ \iffi $wRu \in \mathbf{R}$;

\item $x \in D(w)$ \iffi $(x \in D(w)) \in \mathbf{R}$;

\item $(x_{1}, \ldots, x_{n}) \in V(p,w)$ \iffi $w : p(x_{1},\ldots,x_{n}) \in \mathbf{\Gamma}$.

\end{itemize}
 We now argue that $M$ is a model and satisfies $\fcset$. First, observe that $W \neq \emptyset$ because in the input $\Gamma \cup \Delta \neq \emptyset$, and every bottom-up application of a rule either preserves or adds new labels to its premise(s). Second, it is evident that $R \subseteq W \times W$, and third, since $y \in D(u)$ occurs in $\Lambda$, we know that $D(W)\neq \emptyset$. Fourth, we know that if $(x_{1}, \ldots, x_{n}) \in V(p,w)$, then by the definition of $V$, $w : p(x_{1},\ldots,x_{n}) \in \mathbf{\Gamma}$, and so, by the $\domr$ step of $\prove$, $x_{1} : D(w), \ldots, x_{n} : D(w) \in \mathbf{R}$, showing that $V(p,w) \subseteq D(w)^{n}$ for each $p \in \pred$ or arity $n$ and $w \in W$. Last, it is straightforward to confirm that if $S$, $G(n,k)$, $I_{d}$, $D_{d}$, $C_{d}$, or $N_{d}$ occurs in $\fcset$, then $M$ satisfies the frame condition due to the $\D$, $\sa$, $\idom$, $\ddom$, and $\ned$ steps of $\prove$. Hence, $M$ is a model based on a frame $F \in \mathcal{F}_{\fcset}$.
 
 We now define the assignment $\mu : \var \to D(W)$ such that $\mu(x) = x$ for $x \in D(W)$ and $\mu(y) \in D(W)$ for $y \not\in D(W)$. We now prove the following two claims by mutual induction on the complexity of $\phi$: (1) if $w : \phi \in \mathbf{\Gamma}$, then $M,w,\mu \Vdash \phi$, and (2) if $w : \phi \in \mathbf{\Delta}$, then $M,w,\mu \not\Vdash \phi$. We only argue the atomic and existential cases as the remaining cases are simple or similar.

\begin{itemize}

\item $u : p(\vec{x}) \in \mathbf{\Gamma}$. By the definition of $V$, it immediately follows that $M,u,\mu \Vdash p(\vec{x})$.

\item $u : p(\vec{x}) \in \mathbf{\Delta}$. If $u : p(\vec{x}) \in \mathbf{\Gamma}$, then $\prove$ will halt on $\branch$ at some point due to the $\ax$ step, and thus, $\branch$ will not be infinite, which is a contradiction. Therefore, $u : p(\vec{x}) \not\in \mathbf{\Gamma}$, implying that $M,u,\mu \not\Vdash p(\vec{x})$ by the definition of $V$.

%\item $u : \neg \phi \in \mathbf{\Gamma}$. 

%\item $u : \neg \phi \in \mathbf{\Delta}$.

%\item $u : \phi \lor \psi \in \mathbf{\Gamma}$.

%\item $u : \phi \lor \psi \in \mathbf{\Delta}$.

%\item $u : \Diamond \phi \in \mathbf{\Gamma}$.

%\item $u : \Diamond \phi \in \mathbf{\Delta}$.

\item $u : \exists x \psi \in \mathbf{\Gamma}$. By the $\existsl$ step of $\prove$, the $\existsl$ rule will be applied bottom-up at some point, ensuring that a labeled sequent $\rel', \Gamma' \sar \Delta'$ occurs in $\branch$ such that $z \in D(u) \in \mathbf{R}$ and $u : \psi[z/x] \in \mathbf{\Gamma}$. Hence, $z \in D(u)$ by definition, and by IH, $M,u,\mu \Vdash \psi[z/x]$, showing that $M,u,\mu \Vdash \exists x \phi$.

\item $u : \exists x \phi \in \mathbf{\Delta}$. Let $z$ be an arbitrary element of $D(u)$. Then, $(z \in D(u)) \in \mathbf{R}$ by the definition of $D(u)$. By the $\existsr$ step of $\prove$, the $\existsr$ rule will be applied bottom-up at some point, implying that $u : \psi[z/x] \in \mathbf{\Gamma}$. By IH, $M,w,\mu \not\Vdash \psi[z/x]$, so since $z$ was arbitrarily chosen, it follows that $M,w,\mu \not\Vdash \exists x \psi$.
\end{itemize}
 Let us define $\iota: \lab \to W$ such that $\iota(w) = w$ for $w \in W$ and $\iota(u) \in W$ for $u \not\in W$. By (1) and (2) above, and the definitions of $\mu$ and $\iota$, we can see that $M, \mu, \iota \not\models \Lambda'$, implying that $M, \mu, \iota \not\models \Lambda$. Hence, $\Lambda$ is $\fcset$-invalid.
\end{proof}



